RelateAnything: Real-Time Open-Vocabulary Relation Prediction From Any Inputs

Open-vocabulary detection accepts any class list at inference, and promptable segmentation returns regions without class names: the taxonomy has left the model and become an input. Relation prediction has not. Scene-graph models are still trained and evaluated on the 50 or 56 predicates of one annotation style, their relation head conditioned on object labels and so tied to one detector. Three obstacles explain this, none primarily modelling: no relation corpus is both free-text and verified, a label-conditioned architecture cannot accept a vocabulary it was not trained on, and the standard metric rewards agreement with the training corpus, so a larger vocabulary scores as a regression. We present RelateAnything, a 53M-parameter model taking an image and regions from any source and returning scored relations over a predicate vocabulary supplied at inference as strings. Object labels are never an input, so the region source can change without retraining, and the vocabulary is a bank of text embeddings, not a learned classifier. It runs at 20 ms/frame. Training over 19,103 predicates requires positive-unlabeled supervision and a text encoder that separates antonyms, which contrastive encoders embed at cosine 0.95. To supply the supervision we build RA-4M, 474k images and 4.3M relations over 10,102 free-text predicates, generated against numbered box markers and geometrically verified. To measure it we build OV-SGG-Bench, six axes scored across datasets that the priors standard recall rewards cannot satisfy. On three cross-dataset benchmarks and a fourth zero-shot, RelateAnything has 2.3-3.5x the mean recall of the strongest open-vocabulary method of comparable scale, margins that survive a real detector, and leads a 3B-VLM scene-graph model on both metrics at under 2% of its parameters. In-domain measurement overstates transfer gains ~5x. Model, corpus and benchmark are public.

==> figures/a5_qual_data.tex <==
% GENERATED by paper2/make_a5_qual.py -- do not edit.
% source: runs/judge/qualitative_psg.json; reference: runs/packed/psg/train/meta.json
\def\AqSelection{first 10 images in pack order with >=5 detections, both models emitting >=6 relations, and <=10 distinct boxes referenced; top 10 relations shown per graph}%
\def\AqImgA{figures/a5_qual_1.jpg}%
\def\AqFileA{2316264.jpg}%
\def\AqBoxesA{6}%
\def\AqOursA{\aqrel{1}{dog}{standing on}{5}{dirt}{3.8}\aqrel{0}{cow}{standing on}{4}{grass}{3.8}\aqrel{0}{cow}{standing on}{5}{dirt}{3.8}\aqrel{0}{cow}{standing on}{3}{grass}{3.8}\aqrel{1}{dog}{standing on}{3}{grass}{3.8}\aqrel{1}{dog}{standing on}{4}{grass}{3.8}\aqrel{1}{dog}{looking at}{0}{cow}{5.7}\aqrel{0}{cow}{standing on}{2}{tree}{3.8}\aqrel{0}{cow}{beside}{1}{dog}{2.5}\aqrel{1}{dog}{standing on}{2}{tree}{3.8}}%
\def\AqOursNA{10}%
\def\AqOursBitsA{38.9}%
\def\AqBaseA{\aqon{0}{cow}{on}{5}{dirt}{2.3}\aqon{1}{dog}{on}{5}{dirt}{2.3}\aqon{1}{dog}{on}{3}{grass}{2.3}\aqon{0}{cow}{on}{3}{grass}{2.3}\aqon{0}{cow}{on}{4}{grass}{2.3}\aqon{1}{dog}{on}{4}{grass}{2.3}}%
\def\AqBaseNA{6}%
\def\AqBaseBitsA{13.9}%
\def\AqImgB{figures/a5_qual_2.jpg}%
\def\AqFileB{2316281.jpg}%
\def\AqBoxesB{5}%
\def\AqOursB{\aqrel{4}{banner}{in front of}{1}{sky}{4.6}\aqrel{4}{banner}{in front of}{0}{tree}{4.6}\aqrel{4}{banner}{in front of}{2}{building}{4.6}\aqrel{4}{banner}{in front of}{3}{stop sign}{4.6}\aqrel{1}{sky}{in front of}{0}{tree}{4.6}\aqrel{0}{tree}{beside}{2}{building}{2.5}\aqrel{0}{tree}{beside}{3}{stop sign}{2.5}\aqon{2}{building}{on}{3}{stop sign}{2.3}\aqon{3}{stop sign}{on}{2}{building}{2.3}\aqrel{0}{tree}{standing on}{1}{sky}{3.8}}%
\def\AqOursNB{10}%
\def\AqOursBitsB{36.4}%
\def\AqBaseB{\aqon{0}{tree}{on}{1}{sky}{2.3}\aqon{2}{building}{on}{1}{sky}{2.3}\aqon{4}{banner}{on}{1}{sky}{2.3}\aqon{2}{building}{on}{3}{stop sign}{2.3}\aqon{3}{stop sign}{on}{1}{sky}{2.3}\aqon{3}{stop sign}{on}{2}{building}{2.3}\aqon{4}{banner}{on}{0}{tree}{2.3}\aqrel{2}{building}{beside}{0}{tree}{2.5}\aqon{0}{tree}{on}{2}{building}{2.3}\aqon{0}{tree}{on}{3}{stop sign}{2.3}}%
\def\AqBaseNB{10}%
\def\AqBaseBitsB{23.3}%


==> figures/overview_data.tex <==
% !TEX root = ../main.tex%
% GENERATED by paper2/make_overview.py -- every number and string in%
% figure 1 comes from an artefact under runs/. Do not edit by hand.%
\def\ovImages{474}%
\def\ovRelations{4.3}%
\def\ovPredicates{10{,}102}%
\def\ovRelsPerImg{9.03}%
\newcommand{\ovRegionColours}{%
  \definecolor{ovr1}{HTML}{0B4F8A}%
  \definecolor{ovr2}{HTML}{C2571A}%
  \definecolor{ovr3}{HTML}{0E7C86}%
  \definecolor{ovr4}{HTML}{7A4E9E}%
  \definecolor{ovr5}{HTML}{B3123F}%
  \definecolor{ovr6}{HTML}{148C50}%
  \definecolor{ovr7}{HTML}{D6A21B}%
}%
\newcommand{\ovBoxesOne}{%
  \draw[ovr1, line width=0.6pt] \bxp{0.3107}{0.3366} rectangle \bxp{0.5418}{0.6469};%
  \draw[ovr2, line width=0.6pt] \bxp{0.5572}{0.4389} rectangle \bxp{0.7685}{0.7261};%
  \draw[ovr3, line width=0.6pt] \bxp{0.2315}{0.2739} rectangle \bxp{0.3613}{0.3663};%
  \draw[ovr4, line width=0.6pt] \bxp{0.5330}{0.4092} rectangle \bxp{0.5924}{0.5512};%
  \node[ovbadge, fill=ovr1] at \bxp{0.3107}{0.6469} {1};%
  \node[ovbadge, fill=ovr2] at \bxp{0.5572}{0.7261} {2};%
  \node[ovbadge, fill=ovr3] at \bxp{0.2315}{0.3663} {3};%
  \node[ovbadge, fill=ovr4] at \bxp{0.5330}{0.5512} {4};%
}%
\newcommand{\ovBoxesThree}{%
  \draw[ovr1, line width=0.6pt] \bxp{0.0391}{0.1709} rectangle \bxp{0.3486}{0.9282};%
  \draw[ovr2, line width=0.6pt] \bxp{0.5811}{0.1929} rectangle \bxp{0.9131}{0.4844};%
  \draw[ovr3, line width=0.6pt] \bxp{0.0000}{0.2002} rectangle \bxp{0.9990}{1.0000};%
  \draw[ovr4, line width=0.6pt] \bxp{0.9355}{0.5913} rectangle \bxp{0.9990}{0.8975};%
  \node[ovbadge, fill=ovr1] at \bxp{0.0500}{0.9282} {1};%
  \node[ovbadge, fill=ovr2] at \bxp{0.5811}{0.4844} {2};%
  \node[ovbadge, fill=ovr3] at \bxp{0.1550}{0.9400} {3};%
  \node[ovbadge, fill=ovr4] at \bxp{0.9355}{0.8975} {4};%
}%
\newcommand{\ovCorpusRows}{%
  \ovpanel{1}{\includegraphics[width=\AW cm]{figures/ov_corpus_1.jpg}}{boxes}{\ovBoxesOne}%
  \ovtext{1}{2}{person}{sitting on}{snowboard}{4}{2}{grow}%
  \ovpanel{2}{\includegraphics[width=\AW cm]{figures/ov_corpus_2_masks.jpg}}{masks}{}%
  \ovtext{2}{1}{person}{operating}{land vehicle}{2}{1}{semantic}%
  \ovpanel{3}{\includegraphics[width=\AW cm]{figures/ov_corpus_3.jpg}}{boxes}{\ovBoxesThree}%
  \ovtext{3}{2}{van}{to the right of}{tree}{1}{3}{spatial}%
}%
\def\ovNumRows{3}%
\def\ovGenModel{Gemma\,4}%
\def\ovSegmenter{SAM 2.1}%
\def\ovGenSize{26B}%
\def\ovGenPasses{semantic, grow, spatial}%
\def\ovGenHours{104}%
\def\ovGateRejected{498}%
\def\ovGateRepaired{34}%
\def\ovParams{53}%
\def\ovLatency{20}%
\def\ovDevice{A40}%
\def\ovVocabShipped{243}%
\def\ovVocabTrained{19{,}103}%
\newcommand{\ovVocabList}{%
  \ovvocab{0}{following}%
  \ovvocab{1}{illuminating}%
  \ovvocab{2}{parked by}%
  \ovvocab{3}{wearing}%
  \ovvocab{4}{riding}%
}%
\def\ovVocabListN{5}%
\newcommand{\ovGraphNodes}{%
  \ovgnode{1}{bus}%
  \ovgnode{2}{bus}%
  \ovgnode{3}{building}%
  \ovgnode{4}{street light}%
  \ovgnode{5}{car}%
}%
\newcommand{\ovGraphEdges}{%
  \ovgedge{2}{1}{following}{0.83}%
  \ovgedge{4}{1}{illuminating}{0.81}%
  \ovgedge{5}{3}{parked by}{0.75}%
  \ovgedge{4}{3}{illuminating}{0.64}%
  \ovgedge{1}{5}{passing}{0.61}%
}%
\def\ovNumScored{5}%
\def\ovOursAone{0.3079}%
\def\ovOursAtwo{0.6920}%
\def\ovOursAthree{0.3247}%
\def\ovOursAfour{0.2740}%
\def\ovOursAfive{0.6657}%
\def\ovOursAsix{0.3794}%
\def\ovOursOVS{40.1}%
\def\ovBaseAone{0.1293}%
\def\ovBaseAtwo{0.4621}%
\def\ovBaseAthree{nan}%
\def\ovBaseAfour{0.0404}%
\def\ovBaseAfive{0.4790}%
\def\ovBaseAsix{0.1812}%
\def\ovBaseOVS{11.8}%
\def\ovAfiveOurs{0.67}%
\def\ovAfiveBase{0.48}%


==> tables/a5_pilot.tex <==
% !TEX root = ../main.tex
% GENERATED by paper2/make_tables.py -- do not edit.
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{l}{\sffamily\itshape graph shape, no ground truth and no judge} \\
\sffamily\bfseries model & rel./graph & distinct pred. & modal share & vocab used & at cap \\
\midrule
\ourrow \model{} (v35), vocab = pack & 19.1 & 4.2 & 0.52 & 33 & 91\% \\
OvSGTR \citep{ovsgtr} & 10.3 & 1.7 & 0.85 & 26 & 24\% \\
\midrule
\multicolumn{6}{l}{\sffamily\itshape oracle verdicts, ours against the baseline} \\
\sffamily\bfseries arm & compared & decisive & win rate & longer: win rate ($n$) & equal: win rate ($n$) \\
\midrule
vocab = pack & 143 & 66 & 0.24 & 0.16 (103) & 0.50 (40) \\
\midrule
\multicolumn{6}{l}{\note{controls: scramble accuracy 0.95 (37 decisive of 101), padding resistance 1.00 (10 of 27), primacy 0.42}} \\
\multicolumn{6}{l}{\note{judge Qwen/Qwen2.5-VL-7B-Instruct, 6 votes per comparison, majority 0.67, both presentation orders}} \\
\bottomrule
\end{tabular}

